An extension of Overbeck's attack with an application to cryptanalysis of Twisted Gabidulin-based schemes

In this article, we discuss the decoding of Gabidulin and related codes from a cryptographic point of view, and we observe that these codes can be decoded solely from the knowledge of a generator matrix. We then extend and revisit Gibson and Overbeck attacks on the generalized GPT encryption scheme (instantiated with the Gabidulin code) for different ranks of the distortion matrix. We apply our attack to the case of an instantiation with twisted Gabidulin codes.

==> src/misc.tex <==
\section{To be removed}

\alain{Quel message veut-on faire passer?}

